DiffFit: Visually-Guided Differentiable Fitting of Molecule Structures to a Cryo-EM Map

We introduce DiffFit, a differentiable algorithm for fitting protein atomistic structures into an experimental reconstructed Cryo-Electron Microscopy (cryo-EM) volume map. In structural biology, this process is necessary to semi-automatically composite large mesoscale models of complex protein assemblies and complete cellular structures that are based on measured cryo-EM data. The current approaches require manual fitting in three dimensions to start, resulting in approximately aligned structures followed by an automated fine-tuning of the alignment. The DiffFit approach enables domain scientists to fit new structures automatically and visualize the results for inspection and interactive revision. The fitting begins with differentiable three-dimensional (3D) rigid transformations of the protein atom coordinates followed by sampling the density values at the atom coordinates from the target cryo-EM volume. To ensure a meaningful correlation between the sampled densities and the protein structure, we proposed a novel loss function based on a multi-resolution volume-array approach and the exploitation of the negative space. This loss function serves as a critical metric for assessing the fitting quality, ensuring the fitting accuracy and an improved visualization of the results. We assessed the placement quality of DiffFit with several large, realistic datasets and found it to be superior to that of previous methods. We further evaluated our method in two use cases: automating the integration of known composite structures into larger protein complexes and facilitating the fitting of predicted protein domains into volume densities to aid researchers in identifying unknown proteins. We implemented our algorithm as an open-source plugin (github.com/nanovis/DiffFit) in ChimeraX, a leading visualization software in the field. All supplemental materials are available at osf.io/5tx4q.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January and March 2023

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unix-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> content/02-Relatedwork.tex <==
\section{Background and Related Work}
\label{sec:related-work}

We rely on \ac{Cryo-em} data, so below we first briefly provide essential relevant background. We then describe past work on image registration and model fitting and show how both relate to our own research.

% We rely on \ac{Cryo-em} data, so below we first briefly provide essential relevant background. Then we describe past work on image registration and model fitting and show how both relate to our own research.

\subsection{Brief background}

Structural biology employs various techniques to understand how atoms are arranged in macromolecular complexes, ranging from 60\,kDa (\ie, 4,472 atoms; \href{https://doi.org/10.2210/pdb6NBD/pdb}{PDB 6NBD} \cite{Herzik:2019:HSD}) to 50,000\,kDa (3,163,608 atoms; \href{https://doi.org/10.2210/pdb8J07/pdb}{PDB 8J07} \cite{Walton:2023:ASR}). These techniques are essential for the study of processes in living cells---\ac{Cryo-em} being a particularly powerful one~\cite{Bai2015,MALHOTRA2019Modeling,Lasker2007EMatch}. Using \ac{Cryo-em}, bioscientists can capture images of flash-frozen biological specimens using an electron microscope, preserving their natural structure without the interference of staining or fixing \cite{Chen2023}. These images are then used to construct 3D volumes or maps using the \emph{single particle method}, which aligns thousands of projections from structurally identical molecular instances into a single map (using the Fourier slice-projection theorem) that represents the electron density of the sample, which can be used to infer atom positions within the molecule.

Subsequently, bioscientists must build accurate atomistic or molecular models that match the electron density map obtained from the \ac{Cryo-em} process to gain insight into molecular function and interactions. This process involves mapping or fitting known sub-molecules into their corresponding positions within the map. The objective is to achieve an optimal correspondence between the model and the experimental or simulated volume, revealing the organization of molecules in 3D space, including single molecules, complexes, and the placement of small molecules and ligands into binding sites. Molecular models are available in the Protein Data Bank (PDB, \href{https://www.rcsb.org/}{\texttt{rcsb\discretionary{}{.}{.}org}}), accessible in various formats such as PDB, Crystallographic Information File (CIF), and mmCIF (macromolecular CIF). The fitting is, nowadays, typically achieved through manual placement, alignment, and comparison with the density maps. Due to the manual nature of this process, it is time-consuming and tedious, and can only be performed by expert biologists. To overcome this challenge, researchers have aimed to automate the fitting process in numerous studies, which we review below, focusing on image registration as the foundation and exploring methods to streamline 3D model construction.

\subsection{Image registration and geometric fitting}

The fitting of 3D structures into captured or simulated volumes relates to the problem of image registration in image processing. It entails aligning two images, originating from the same or different modalities, within a shared reference frame \cite{Hill2001, Fu2020}. This process involves feature extraction, determining transformations, and assessing accuracy through metrics.
Scale-invariant features from images~\cite{Lowe2004}, for example, can facilitate matching across diverse views, despite significant distortions or variations. This process involves detecting invariant keypoints using the difference-of-Gaussian function, determining locations and scales, assigning directions based on local gradients, and measuring gradients within selected scales around each keypoint. Extracted features are stored in a database, enabling them to be matched with new images using fast nearest-neighbor algorithms, with applications including object recognition. 

Among many applications of the process, physicians rely on various imaging modalities to diagnose patients, each capturing images with differing orientations. Image registration addresses this variability by aligning images within a unified frame by optimizing parameters such as orientation and translation. 
Medical image registration is an active research area encompassing diverse methods, including techniques based on cross-cor\-re\-la\-tion \cite{Didon1995,Malinsky2013} and mutual information \cite{Pluim2003,Mattes2003,Thevenaz2000,Klein2009}.
%
Shang \etal~\cite{SHANG2006}, for example, introduced a method for medical image registration using \ac{pca} neural networks to extract feature images and compute rotation angles and translation parameters by aligning the first principal directions and centroids in a simple and efficient way. For complex spatial transformations, another recent approach~\cite{arora2024integration} uses Kernel \ac{pca} and Teaching-Learning-based optimization (TLBO) for multi-modal image registration. 
%
Similar to these methods, transformations and alignments must be determined to fit the atomistic model into a volumetric map. We can thus also use optimization techniques in \ac{Cryo-em} map fitting to refine the fit and optimize parameters such as orientation and translation---which is demonstrated in our work. The major difference compared to image registration is that, in our workflow, we fit two different data representations and one is a sub-part of the whole that is potentially present at multiple locations in the target volume.

Model-to-data fitting, which is necessary for \ac{Cryo-em} data, has also been investigated in depth in computer graphics and pattern recognition~\cite{Reddy2020Differentiable,K2018Direct}, with applications in architectural geometry, virtual and augmented reality, robotics, and various other fields \cite{Falk2023,Agnes2018Spline,kou2024adaptive,Yeh2011Template} in addition to structural biology. The key challenges in geometric fitting include accuracy, efficiency, robustness, and usability of the fitting module~\cite{Agnes2018Spline,kou2024adaptive}. Structural biology, in contrast, has different challenges, such as noisy data, non-geometric shapes, and large data sizes so that geometric fitting methods are not directly applicable.

Yet our \acronym algorithm still relates to techniques from computer graphics and pattern analysis. The differentiable compositing technique proposed by Reddy \etal \cite{Reddy2020Differentiable}, in particular, offers valuable insights into addressing fitting challenges as well as manipulating and understanding image patterns. With \emph{differentiable compositing} we can handle patterns effectively, outperforming state-of-the-art alternatives in pattern manipulation \cite{Zhou2018Nonstationary,Shaham2019SinGANICCV}. Reddy \etal's ~\cite{Reddy2020Differentiable} discovers complex patterns by aligning elements with their own position and rotation, and facilitates refinement based on similarity to the target for precise adjustment. In addition, Reddy \etal use a multi-resolution pyramid---relevant for handling the multi-resolution volumetric data in our domain. Their method~\cite{Reddy2020Differentiable}, however, is restricted to certain pattern types, requires manual element marking, and may not always find the best solution, leading to orientation errors and missed elements. Nevertheless, our solution is built on top of their differentiable compositing.

Another approach, spline surface fitting \cite{Agnes2018Spline}, enhances the smoothness in aircraft engine geometry reconstruction by concurrently approximating point and normal data, ensuring boundary smoothness and optimal convergence, while exploring norm-like function effects on error measurement. Another recently proposed adaptive spline surface fitting method~\cite{kou2024adaptive}, supported by empirical evidence, employs surface meshes for high-precision CAD applications. The reliance of this approach on control meshes, however, limits its applicability to irregular topologies and compromises the preservation of sharp features. All these methods have common objectives and tasks such as similarity measures, pattern matching, fitting, and geometric transformations; thus, they can serve as motivation and a starting point toward our goals in structural biology. Structural biology data often consists of large, complex structures without regular shapes like CAD models or easy representations in geometric meshes with smooth surfaces, however the aforementioned methods are not directly applicable to our data.
 
\subsection{Fitting in structural biology}

Existing fitting methods for structural biology can be broadly categorized into manual, semi-automated, and automated approaches, each with their own advantages and challenges when used for aligning molecular models with \ac{Cryo-em} density maps. Manual or semi-automated methods involve human intervention, yet they provide control and precision---which is particularly beneficial in the structural analysis of complex datasets or when specific adjustments are needed for accuracy. For example, UCSF ChimeraX~\cite{pettersen2004ucsf}, a popular tool for molecular manipulation and visualization, includes the \emph{fitmap} technique \cite{Thomas2007}. It suggests multiple possible placements of the atomistic model on the density map and then asks the user to make the final decision. The fitting process alternates between rigid-body rotation and gradient descent translation, maximizing alignment between the atomic model and density data by optimizing the sum of density values. 
Nonetheless, all of these manual or semi-automatic approaches are time-consuming and require a significant level of expertise.

To tackle this challenge and to automate the fitting process, researchers have developed methods that rely on deep learning (DL) \cite{Xu2019,Terwilliger2018,Wang2020}. $A^2$-Net by Xu \etal \cite{Xu2019}, for example, uses DL to accurately determine amino acids within a 3D \ac{Cryo-em} density volume. It employs a sequence-guided Monte Carlo Tree Search (MCTS) to traverse candidate amino acids, considering the sequential nature of amino acids in a protein. The authors divide the molecular structure determination problem into three subproblems: amino acid detection in the density volumes, assignment of atomic coordinates to determine the position of each amino acid, and main chain threading to resolve the sequential order of amino acids that form each protein chain. A remarkable speed improvement is also demonstrated by Xu \etal, being 100 times faster to find solutions at runtime than existing methods \cite{frenz2017rosettaes,wang2015novo}, and achieving a high accuracy of $89.8\%$. In addition, they introduced the $A^2$ dataset with 250,000 amino acids in 1,713 \ac{Cryo-em} density volumes, with a resolution of 3 $A^{\circ}$, pioneering automated molecular structure determination training benchmarks.

Another recent method by Mallet \etal, CrAI, uses machine learning (ML) to find antibodies in cryo-EM densities \cite{Mallet2023}. The authors formulate the objective as an object detection problem, using the structural properties of Fabs (Fragment antigen-binding) and VHHs (single-domain antibodies). Furthermore, DeepTracer \cite{Pfab2021} is a fully automated DL-based method designed to determine the all-atom structure of a protein complex using its high-resolution \ac{Cryo-em} map and amino acid sequence. This method employs a customized deep convolutional neural network primarily for the precise prediction of protein structure, including the locations of amino acids, backbone, secondary structure positions, and amino acid types. The reprocessed \ac{Cryo-em} maps are the input to the neural network, which transforms the output into a protein structure. 
Despite yielding accurate outcomes, the resulting atomistic structures may exhibit geometric issues, local fit to map discrepancies, misplaced side chains, or errors in tracing and/or connectivity.
All DL-based techniques require a substantial amount of time for training (as opposed to the runtime) and rely on large training datasets of \ac{Cryo-em} volumes and manually fitted sub-molecules---based on this, we do not employ DL approaches.

An alternative to DL is map-to-map alignment, which is used to accurately align 2D or 3D maps to facilitate comparison and analysis of spatial structures or features within the maps. CryoAlign \cite{he2024} is a \ac{Cryo-em} density map alignment method that achieves a fast, accurate, and robust comparison of two density maps based on local spatial feature descriptors. This approach involves sampling the density map to generate a point cloud representation and extracting key points by clustering based on local properties. CryoAlign then calculates local feature descriptors to capture structural characteristics, reducing the number of points considered, and improving efficiency. By employing a mutual feature-matching strategy, CryoAlign establishes correspondences between keypoints in different maps and uses iterative refinement to enhance alignment. A combination of fast rotational matching search based on spherical harmonics and translational scans \cite{garzon2006} yields accurate fitting results in seconds up to a few minutes. This ADP\_EM approach is particularly reliable in fitting X-ray crystal structures to low-resolution density maps, with reduced docking times and maintaining a thorough 6D exploration with fine rotational sampling steps to find valid docking solutions.

In our work, we design a differentiable optimization method for fitting atomistic structures into volumetric data, with the goal of precise fitting with computation that is rapid enough to be applicable in semi-automatic fitting in the standard tool ChimeraX. For this purpose, we use the PyTorch capabilities for GPU parallel computing, trilinear interpolation sampling in volumetric data, and auto differentiation.




==> content/03-Method.tex <==
\section{Method}
\label{sec:method}
\begin{figure*}[!t]
  \centering
  \includegraphics[width=\linewidth]{figs/difffit_scheme.PNG}
  \caption{\acronym workflow. The target \ac{Cryo-em} volume and the structures to be fit on the very left serve as input and are passed to the novel volume processing, followed by the differentiable fitting algorithm. 
  The fitting results are then clustered and inspected by experts, who may zero out voxels corresponding to the placed structures and feed the map back iteratively as input for a new fitting round until the compositing is finished.}
  \label{fig:method_overview}
\end{figure*}

This section describes the proposed approach by explaining the process of differentiable structure fitting before demonstrating how it can be used for visually guided fitting. After discussing these conceptual aspects, the implementation is briefly detailed.

\subsection{Differentiable structure fitting}
Given a \ac{Cryo-em} map, the domain practitioners---bioscientists---do not know the precise location and orientation parameters governing where and how protein substructures fit together. For some regions in the map, bioscientists may not even know which protein subunits should be present. Our goal is to develop a new approach to address these domain tasks. In cases where bioscientists are highly confident of the presence of certain protein subunits in the map, the proposed technique aids in the identification of their respective placement parameters. For regions with unknown protein subunits, the task of the proposed technique is to identify potential protein subunit candidates that best fit the \ac{Cryo-em} map region from a large database. 

\subsubsection{Inspiration and approach overview}

We base our approach on the mentioned 2D differentiable compositing approach by Reddy \etal \cite{Reddy2020Differentiable}, which discovers the pattern structure from wallpaper-like textures containing repetitive patterns comprising elementary patches. We first review their approach, before we describe how we build up our solution on top of their technique. In their case, given a 2D image, a composite of multiple small element patches, the task is to identify the number of occurrences and placement parameters for each existing patch. The parameters include the type of patch (out of several known patches) and the position, orientation, and depth. Their solution distributes tens to hundreds of patches in the image and uses the differentiable optimization method to translate and reorient patterns such that they correspond to the appearance of those in the input wallpaper image. Each instance $E_i$ (out of total number of $\omega$ instances) of a pattern is stored in a layer $J_i$ for each patch instance by sampling from that patch, considering the translation, rotation, and patch-pattern type probability:\vspace{-1ex}
%
\begin{equation}
J_i(\mathbf{x})=f_t\left(\mathbf{x}, E_i\right)=\frac{1}{\sum_{k=1}^o e^{t_i^k}} \sum_{j=1}^o e^{t_i^j} h_j\left(R_{\theta_i}^{-1}\left(\mathbf{x}-\mathbf{c}_i\right)\right)
\end{equation}\vspace{-1ex}

\newlength{\lineskiplimitbackup}%
\setlength{\lineskiplimitbackup}{\lineskiplimit}%
\setlength{\lineskiplimit}{-\maxdimen}%
\noindent where $f_t\left(\mathbf{x},E_i\right)$ represents a differentiable function using the expected value over the patch-pattern type probabilities stored in a tuple $\mathbf{t}$ representing all $o$ patch patterns, softmax $e^{t_i^k}/\sum_{k=1}^m e^{t_i^k}$ over the type logits defines the patch-pattern type probabilities, $h_j$ denotes the image patch sampler function, $\mathbf{x}$ represents the image location, $\mathbf{c}_i$ is the center location of patch element $E_i$, and $R_{\theta_i}^{-1}$ indicates the inverse of a $2\times2$ matrix rotation with angle $\theta_i$.
 
\setlength{\lineskiplimit}{\lineskiplimitbackup}%

The solution image results from compositing all instances using the $f_c$ compositing function so that each known patch-pattern type is present multiple times with various positional parameters. Patches can overlap other patches, leading to partial or full occlusion of a certain pattern, which is characterized by $v_i(\mathbf{x}), v \in \{0,1\}$, which is the visibility of layer $i$ at image location $\mathbf{x}$:\vspace{-1ex}
\begin{equation}
I(\mathbf{x})=f_c\left(\left\{J_i(\mathbf{x})\right\}_i\right)=\sum_{i=0}^\omega J_i(\mathbf{x}) v_i(\mathbf{x}).
\end{equation}
This solution image is compared to the input image in an optimization, where the parameters of all patch instances are updated in every iteration. Then, the so\-lu\-tion image becomes increasingly similar to the in\-put image. Reddy \etal defined the $L^2$ distance loss $L_d$ for the optimizer as follows:\vspace{-1ex}
\begin{equation}
L_d(A, I)=\frac{1}{P} \sum_{p=1}^P\left\|A\left(\mathbf{x}_p\right)-I\left(\mathbf{x}_p\right)\right\|_2^2
\end{equation}
where the sum is over the number of all pixels $P$ in the image, $A$ denotes the input image, and $I$ indicates the composited solution image.
Then, optimal elements $\mathcal{E}^*$ are determined by minimizing  loss $L_d$ over the entire set of elements $\mathcal{E} = \{E_0, .., E_\omega\}$
:\vspace{-1ex}
\begin{equation}
\mathcal{E}^*=\underset{\mathcal{E}}{\arg \min } ~L_d(A, f_c(\mathcal{E})) .
\end{equation}

\begin{figure*}[t]
  \centering
%\[ \begin{array}{cccccc} 
	\setlength{\subfigcapskip}{-2.5ex}
  \subfigure[\hspace{\columnwidth}]{\label{fig:clustering_filtering:a}\includegraphics[height=4cm]{figs/fig3/3_1.png}}\hfill% &
  \subfigure[\hspace{\columnwidth}]{\label{fig:clustering_filtering:b}\includegraphics[height=4cm]{figs/fig3/3_2.png}}\hfill% &
  \subfigure[\hspace{\columnwidth}]{\label{fig:clustering_filtering:c}\includegraphics[height=4cm]{figs/fig3/3_3.png}}\hfill% &
  \subfigure[\hspace{\columnwidth}]{\label{fig:clustering_filtering:d}\includegraphics[height=4cm]{figs/fig3/3_4.png}}\hfill% &
  \subfigure[\hspace{\columnwidth}]{\label{fig:clustering_filtering:e}\includegraphics[height=4cm]{figs/fig3/3_5.png}}\hfill% &
  \subfigure[\hspace{\columnwidth}]{\label{fig:clustering_filtering:f}\includegraphics[height=4cm]{figs/fig3/3_6.png}}\vspace{-2ex}% \\
  %(a) & (b) & (c) & (d) & (e) & (f) \\ 
%\end{array} 
%\]
  \caption{Clustering and filtering: (a) target volume, (b) atom coordinates of the source structure, (c) positions of 1000 fit results (dots are clustered, hiding the number of results), (d) 1000 instances of the structure, (e) positions of 1000 fit results with the transparency level set based on an exponential scaling of the correlation metric (two clusters stand out), and (f) instances of the structure at these two clusters.}
  \label{fig:clustering_filtering}
\end{figure*}

The patch-pattern fitting problem in the work by Reddy \etal is similar to the problem in this work in the sense that element instances are composited into a scene in both cases. However, the differentiable compositing approach in their work cannot be directly applied to the structural biology domain to solve the protein fitting problem for the following reasons:
\begin{enumerate}[noitemsep]
    \item The pattern image and element patches are defined in 2D with layers, whereas the \ac{Cryo-em} map and protein subunits are defined in 3D. 
    \item The pattern image and element patches are of the same representation (i.e., 2D grid data), whereas the \ac{Cryo-em} map and protein subunits are of different representations: one is a 3D volume and the other is a set of atom coordinates that can be considered a point cloud. 
    \item The instance patches in differentiable compositing are all the same size, whereas the protein subunits differ in the number of atoms.
    \item Differentiable compositing expects the patches to overlap, whereas protein subunits do not spatially overlap. 
    \item Finally, 1000 layers of 2D images can fit into the current GPU memory, whereas 1000 3D volumes cannot with the currently available GPU memory.
\end{enumerate}

Initially, we attempted to align our problem better with differentiable compositing by first \emph{simulating} a \ac{Cryo-em} map from the atomistic point cloud of the protein model and then fitting the simulated map to a target map. That way the representational discrepancy (see reason (2) above) is eliminated. That approach, however, was only successful for trivial cases, while for real-world scenarios it frequently fell into local minima. Interested reader will find exemplary volume-only based molecular fitting videos in supplementary material at \href{https://osf.io/5tx4q/}{\texttt{osf.io/5tx4q}}.

Initially, we attempted to eliminate any representational discrepancy (see Reason 2) by first \emph{simulating} a \ac{Cryo-em} map from the atomistic point cloud of the protein model and then fitting it to a target map. However, that approach was only successful for trivial cases, whereas the solution frequently fell into local minima for real-world scenarios. (Exemplary volume-only based molecular fitting videos are available in the supplementary material at \href{https://osf.io/5tx4q/}{\texttt{osf.io/5tx4q}}).

Driven by the successful fitting cases from many experiments, we gradually built several novel strategies on top of differentiable compositing that effectively address molecular structure fitting. 
Most notably, we address the substantially higher complexity of our scenario based on the knowledge, experience, and deep insight of the target audience: bioscientists. Our solution is thus based on a human-in-the-loop strategy, and we propose a fast and robust visual analytics approach, \acronym, with two main steps: (1) an automated excessive molecular fitting and (2) visual inspection and filtering of the fitted results by bioscientists. These two consecutive steps are building blocks of a visual analytic feedback loop, where multiple proteins are iteratively composited to fit the underlying \ac{Cryo-em} volume. 


\autoref{fig:method_overview} schematically presents the proposed \acronym workflow. 
First, an excess number of all compositing molecules is seeded in the volume scene. If simultaneously fitting all molecules exceeds the available GPU memory, the molecules are sorted by atom count and partitioned into batches. Then, the batches of molecules are fit in several iterations in descending atom-count order. 
This fitting relies on a novel loss function that calculates the average density value from the densities sampled by each atom. The differentiable property of the proposed fitting scenario allows optimization based on the gradient descent. In addition, each fit is associated with a numerical value that characterizes the fit quality. For this purpose, a simulated \ac{Cryo-em} map of each fitted molecule is created, and the correlations of the simulated densities are calculated using the real \ac{Cryo-em} map densities. Then, the fitting results are collected and clustered based on positional and orientational parameters. For each cluster, one representative fit---the fit with the highest correlation value--- is selected. Then, the clusters are sorted by their representative correlations and interactively visualized in ChimeraX to allow bioscientists to inspect the solutions. Once a given molecular placement is verified, molecule placements in the respective regions are disabled in the following iterations by setting voxels covered by the molecular fit in the \ac{Cryo-em} map volume to zero. Thus, the successful placements are gradually erased from the map, forcing the following placements to search for a fit in nonzero volume locations. Once the feedback update in the map is completed, the next fitting iteration is performed with another molecular structure. This workflow pattern is repeated until the map has nearly all voxels zeroed out, and the entire sub-unit placement of the complex molecular structure is complete. The details of \acronym are detailed in the following order: (1) sample one coordinate, (2) fit one placement of one molecule, (3) fit multiple placements of one molecule, and (4) fit multiple placements of multiple molecules.


\subsubsection{Sampling of one coordinate}

Because the task is to determine the optimal alignment of an atomistic molecular structure to the reconstructed \ac{Cryo-em} volume map, the optimal fit characterized by two rigid-body transformation parameters is determined: a translational offset $\mathbf{p}$ and a rotation. The rotation is represented by a quaternion $\mathbf{q}$ or its corresponding rotation matrix $M_{\mathbf{q}}$. The position $\mathbf{x}_{i}$ corresponds to the center point of an atom $i$ in the molecular subunit. Every atom position in one subunit is transformed according to the rotation and translational offset to calculate the fit:
\begin{displaymath}
T(\mathbf{x}_i) = M_{\mathbf{q}} \cdot \mathbf{x}_i + \mathbf{p}.
\end{displaymath}

A density value $D$ of the atom to be placed at position $T(\mathbf{x}_i)$ is sampled from a scalar volume $V$ using trilinear interpolation ($S$) as follows: 
\begin{displaymath}
D(T(\mathbf{x}_i)) = S (T(\mathbf{x}_i), V).
\end{displaymath}

\begin{figure*}
	\centering
	\includegraphics[width=\textwidth,height=.5\textwidth]{figs/Viewer.png}
	\caption{Visual browser based on ChimeraX. The target volume on the left is overlaid with a fitted molecule corresponding to the selected fit result in the table on the right (clustered fits, each row is the representative placement with the highest correlation from that cluster). After inspection, users can save the placement and select ``Simulate volume'' and ``Zero density'' to zero out the corresponding voxels from the target volume.}
	\label{fig:visual-browser}
\end{figure*}

\subsubsection{Placement of one molecule (or one subunit)}

An initial loss function $L$ is formulated to determine the best $\mathbf{p}$ and $\mathbf{q}$ parameters. This function provides the minimum negative average density per atom for a molecular subunit with $N$ atoms that form the set $\mathbf{X}_m$ of all atom center points T($\mathbf{x}_i) \in \mathbf{X}_m$ for a particular molecular subunit $m$:
\begin{equation}
L(\mathbf{p}, \mathbf{q}, \mathbf{X}_m, V) = - \left( \frac{1}{N} \sum_{i}^N D(T(\mathbf{x}_i)) \right) = - \frac{1}{N} \sum_{i}^N S(M_\mathbf{q} \cdot \mathbf{x}_{i} + \mathbf{p}, V). 
\end{equation}

The gradient of the differentiable formulation is calculated and used withthe Adam optimizer for the optimization \cite{Kingma:2017:AMS}.
Although the Adam optimizer is known for robustness with respect to local minima, the initial loss function formulation frequently leads to a local minimum (i.e., a place that is not optimal for the molecule in the map but from which the optimizer cannot find a better solution in the parameter-space neighborhood). Local minima are a common, severe problem that also manifests in the functionality of the most commonly used tools for molecular subunit fitting (e.g., fit-in-map feature in ChimeraX). Thus, several strategies are introduced  to form a novel loss function, making \acronym more robust.

The first strategy that substantially contributes to a good fitting performance is \textbf{filtering the input \ac{Cryo-em} map volume} $V$. The volume values are set based on a user-specified minimal threshold and a minimum size of connected voxels that form a cluster. All voxels with a density value less than a given threshold are detected and set to zero. The size of the connected voxel cluster after thresholding must be greater than the cluster size hyperparameter. Otherwise, all the voxels in that cluster are set to zero. This step leads to the filtered volume $V_F$ and ensures that only relevant volume regions are considered for fitting, improving the focus and efficiency of the algorithm. Then, the filtered values are normalized to $[0, 1]$---a typical practice in learning and optimization approaches---, leading to a volume $\hat{V}_F$. This approach is essential for controlling the magnitude of the calculations that lead to the loss function and the settings of the hyperparameters in the workflow.

\setlength{\lineskiplimit}{-\maxdimen}%
A series of convolution iterations were applied to the target volume, capturing each smoothing as a separate volume, to accomodate the noise and variability in biological datasets. This iterative convolutional smoothing leads to an array of volumes, and each volume is used in the fitting process. This \textbf{multi-resolution approach} enhances the robustness of the fitting process by mitigating the impact of noise and data irregularities. 
Empirically, a 10-ele\-ment array of increasingly smoothed volumes, iteratively filtered with a Gaussian smoothing kernel, performs well. The size of this array is a hyperparameter allowing users to control it. Laplacian smoothing was also applied, leading to unsatisfactory performance. The nonsmoothed volume is denoted as $\hat{V}_{F}^{G_0}$, and the recurrent formulation of the iterative convolution smoothing is expressed as follows:\vspace{-1ex}
\begin{displaymath}
\hat{V}_F^{G_n} = \hat{V}_F^{G_{n-1}} * G_n.
\end{displaymath}

\setlength{\lineskiplimit}{\lineskiplimitbackup}%

\setlength{\lineskiplimit}{-\maxdimen}%
A third adaptation applied to the initial fitting process is a stricter penalization of a mismatch. If an atom center is placed in the \ac{Cryo-em} map volume but outside the extent of the molecular target structure (i.e., outside of the target \emph{footprint}), the target density would normally be zero. These regions are assigned a \textbf{negative value} to discourage such misalignments further. After smoothing, for voxels with a density value of zero, the zero is replaced with a negative value. 
The negative values were varied or a smooth gradient of negative values was created, but a constant value of $-0.5$ performs well outside the molecular footprint in the map. However, this value is as a tunable hyperparameter. The resultant volume is denoted by $\hat{V}_{F_{-c}}^{G_n}$, where $-c$ is the negative constant value. Finally, the loss function formulation is updated with a volume smoothed after $j$ iterations as follows:\vspace{-1ex}
\begin{displaymath}
L(\mathbf{p}, \mathbf{q}, \mathbf{X}_m, \hat{V}_{F_{-c}}^{G_j}).
\end{displaymath}

\setlength{\lineskiplimit}{\lineskiplimitbackup}%

Each fit is weighted with a multiresolution volume-array element $w_j$ for $n$ resolutions, and all the multiresolution components are summed to form the final loss function for one $\mathbf{p}$ and $\mathbf{q}$ pair:\vspace{-1ex} 
\begin{equation}
L_m([p, q]) = \sum_{j=1}^{n} w_j \cdot L(\mathbf{p}, \mathbf{q}, \mathbf{X}_m, \hat{V}_{F_{-c}}^{G_j}).
\end{equation}

\setlength{\lineskiplimit}{-\maxdimen}%
The position offset $\mathbf{p}$ and the rotation quaternion $\mathbf{q}$ must be initialized to start the optimization. On a unit sphere, $N_\mathbf{q}$ points  are uniformly sampled and converted into quaternions to be applied for each offset position. Instead of uniformly sampling positions from the volume bounding box (as in ChimeraX), $N_\mathbf{p}$ positions are uniformly sampled from the positive voxels in the filtered and normalized volume $\hat{V}_{F_{-c}}$. 
This \textbf{data-adaptive initialization} increases the success rate by a factor of two by searching from $N_\mathbf{q} \cdot N_\mathbf{p}$ initial placements, compared to the traditional initialization of ChimeraX. 

\setlength{\lineskiplimit}{\lineskiplimitbackup}%

\subsubsection{Fitting multiple placements of one molecule}

Next, GPU parallelization is employed to optimize all $N_\mathbf{q} \cdot N_\mathbf{p}$ pairs of $[\mathbf{p}, \mathbf{q}]$ of the molecule with atoms $\mathbf{X}_m$ in one loss function to determine fits for multiple copies of a single molecule $m$:\vspace{-1ex} 
\begin{equation}
L_{par}(m) = \sum_{k=1}^{N_\mathbf{q} \cdot N_\mathbf{p}} L_m([\mathbf{p}_k, \mathbf{q}_k]).
\end{equation}

\subsubsection{Fitting multiple placements of multiple molecules}


Finally, all subunit molecules have different numbers of atoms; thus, parallelizing the treatment of multiple molecules without overhead on the array padding of zeros is challenging. Usually, the $N_\mathbf{q} \cdot N_\mathbf{p}$ initial placements of $\mathbf{X}_m$ atoms would result in a total number of sampling operations higher than the total number of GPU threads;therefore, different subunit molecules are processed sequentially in a \texttt{for} loop and form an overall loss function for $M$ molecules as follows:\vspace{-1ex}
\begin{equation}
L_{all} = \sum_{l=1}^{M} L_{par}(l).
\end{equation}

\subsubsection{Quantify the fit quality}

Sampling from the molecule in the simulated volume obtains a weight for each atom coordinate, which is $ W(\mathbf{x}) = S (\mathbf{x}, V_{sim})$. Then, for all atoms in a molecule, two vectors can be formed, a sampled density vector $ \mathbf{D} = [D(\mathbf{x}_1), D(\mathbf{x}_2), ..., D(\mathbf{x}_N)] $ from the target volume and a weight vector $ \mathbf{W} = [W(\mathbf{x}_1), W(\mathbf{x}_2), ..., W(\mathbf{x}_N)] $ from the simulated volume. Then, three alignment metrics can be calculated: the mean overlap $\mu$, correlation $\rho$, and  correlation about the mean $\rho_\mu$ as follows:
\begin{displaymath}
\mu = \frac{\mathbf{D} \cdot \mathbf{W}}{N}
\end{displaymath}

\begin{displaymath}
\rho = \frac{\mathbf{D} \cdot \mathbf{W}}{|\mathbf{D}| |\mathbf{W}|}
\end{displaymath}

\begin{displaymath}
\rho_\mu = \frac{(\mathbf{D} - D_\mu) \cdot (\mathbf{W} - W_\mu)}{|\mathbf{D} - D_\mu| |\mathbf{W} - W_\mu|}
\end{displaymath}
where the subtraction operator subtracts the scalar average densities $D_\mu$ and $W_\mu$ from each component of the sampled density vectors. In ChimeraX, bioscientists use these quality metrics during the interactive assessment, which is described next.

\subsection{Visually guided fitting}
A critical aspect of the post-processing of \acronym involves clustering and sorting the fitting results to facilitate user-guided selection and refinement. After the optimization phase, the algorithm generates a vast array of potential fits, characterized by their translation and rotation parameters. A clustering algorithm is applied to group the fitting results based on their spatial and orientational similarity to manage this abundance of data and facilitate efficient exploration of the results (\autoref{fig:clustering_filtering:c}, (e)).

Each cluster represents a set of closely related fits, suggesting a consensus regarding the position and orientation of the fitted structure in the target volume. These clusters are sorted based on a defined metric, such as the overall density overlap or correlation coefficient, ensuring that the most promising fits are prioritized for user review. This hierarchical organization allows researchers to quickly identify the most accurate and relevant fitting results, streamlining the analysis process.

An interactive visual browser was created as a comprehensive visualization tool to present the sorted clusters in a user-friendly format to further assist in exploring the fitting results (\autoref{fig:visual-browser}). This browser displays critical metrics for each cluster, including the average correlation coefficient, density overlap, and consensus error measure, providing a quick overview of the quality and relevance of each cluster. The browser also allows users to select a cluster and visually inspect the fitting results in the 3D context of the target volume. This interactive exploration is crucial to assess the fit quality in complex \ac{Cryo-em} map regions, where subtle differences in position or orientation could substantially influence the biological interpretation of the results.

An innovative feature of the proposed approach is the ability to refine the fitting process iteratively by selectively excluding already-placed molecule densities. Once a bioscientist selects a cluster and verifies (or multiple fits)  as accurate, the corresponding density in the target volume can be \emph{zeroed-out}, removing the volume region from further consideration in the following fitting process. This step is crucial for complex volumes with multiple closely situated structures because it prevents the algorithm from repeatedly fitting structures to the same volume region and reduces false positives when fitting the remaining region. 

 Thus, users can progressively shrink the target volume by iteratively fitting and zeroing out densities and isolating and identifying individual structures in a dense or complex dataset. This iterative refinement approach ensures that the fitting process is guided by the algorithm optimization and the expert knowledge and visual assessment of the user, leading to more accurate and biologically meaningful results. 

The resulting visually guided fitting framework enhances the \acronym algorithm by integrating clustering, sorting, and interactive exploration tools. These features enable users to filter through large datasets of fitting results, identify the most promising fits, and iteratively refine the fitting process efficiently based on a visual assessment. The combination of automated optimization with user-guided inspection and filtering addresses the challenge of accurately fitting molecular subunit structures in volumetric data. 


==> content/04-Use_cases.tex <==
\section{Use Case Scenarios}

\acronym was designed with its advanced fitting algorithms and integration with visualization tools to address a range of challenges in structural biology. Thus, three key scenarios were explored where \acronym can be particularly effective, demonstrating its versatility and potential.

\subsection{Scenario 1: Fit a single structure}



\begin{figure}
     \centering
     %\begin{subfigure}[b]{0.3\linewidth}
         %\centering
         \subfigure[Source structure.]{\label{fig:use_scenario_1_structure}\includegraphics[width=0.32\columnwidth]{figs/use_case_1_1.png}}\hfill%
         %\caption{Source structure}
         %\label{fig:use_scenario_1_structure}
     %\end{subfigure}
     %\hfill
     %\begin{subfigure}[b]{0.3\linewidth}
         %\centering
         \subfigure[Target map.]{\label{fig:use_scenario_1_map}\includegraphics[width=0.32\columnwidth]{figs/use_case_1_2.png}}\hfill%
         %\caption{Target map}
         %\label{fig:use_scenario_1_map}
     %\end{subfigure}
     %\hfill
     %\begin{subfigure}[b]{0.3\linewidth}
         %\centering
         \subfigure[Fitting result.]{\label{fig:use_scenario_1_result}\includegraphics[width=0.32\columnwidth]{figs/use_case_1_3.png}}\vspace{-2ex}
         %\caption{Fit result}
         %\label{fig:use_scenario_1_result}
     %\end{subfigure}
        \caption{Fitting a single structure for \href{https://doi.org/10.2210/pdb8JGF/pdb}{8JGF} \cite{Guo:2023:HAP}.}\vspace{2ex}
        \label{fig:use_scenario_1}
\end{figure}

The most straightforward application of \acronym is fitting a single atomistic structure to a target volumetric map, as illustrated in \autoref{fig:use_scenario_1}. This scenario is common in cases in which an already-resolved protein structure or a predicted structure must be placed in a newly reconstructed volume captured via \ac{Cryo-em} for further refinement.

In this scenario, the optimization of \acronym efficiently determines the optimal position and orientation of the protein (\autoref{fig:use_scenario_1_structure}) in the volume (\autoref{fig:use_scenario_1_map}). The entire fitting process is automatic, removing the prerequisite of manually placing the structure at an approximate orientation close to the final optimal one. 
The interactive visually guided inspection process allows researchers to verify the fit (\autoref{fig:use_scenario_1_result}), applying their expertise to ensure biological relevance and accuracy. The successful hit rate and computation times in \autoref{table:fit_single} are reported and compared them with the current solution in ChimeraX for four recently published structures, where each structure was fitted 1000 times to obtain reliable results. The reported performance values are based on a workstation using a Nvidia RTX 4090 GPU for the \acronym part and a single thread on an AMD Ryzen Threadripper PRO 3995WX 2.70 GHz for the ChimeraX fitmap command.

\begin{table}[t]
\caption{Performance results for fitting a single structure. C stands for ChimeraX, D stands for \acronym; Gain = D/C for Hit and C/D for Time.\vspace{-1ex}}
\begin{tabu}{@{}lllllll@{}}
\toprule
Structure & C Hit & D Hit & Gain & C Time  & D Time  & Gain \\
\midrule
\href{https://doi.org/10.2210/pdb8JGF/pdb}{8JGF} \cite{Guo:2023:HAP} & 11    & 380   & 35\texttimes   & 0:38:57 & 0:00:12 & 195\texttimes  \\
\href{https://doi.org/10.2210/pdb8X79/pdb}{8X79} \cite{Wang:2024:MRA} & 1     & 292   & 292\texttimes  & 0:30:33 & 0:00:14 & 131\texttimes  \\
\href{https://doi.org/10.2210/pdb8GAM/pdb}{8GAM} \cite{Hu:2024:EAI} & 3     & 396   & 132\texttimes  & 1:31:37 & 0:00:14 & 393\texttimes  \\
% 1GRL \cite{LUDTKE:2001:SPR,Braig:1994:CSB} &       &       &      &         &         &      \\
\bottomrule
\end{tabu}
\label{table:fit_single}
%
%\vspace{.5ex}C stands for ChimeraX, D stands for \acronym; Gain = D/C for Hit and C/D for Time. %\todo{[add last line RL: if time permits; otherwise remove]}
\end{table}


\subsection{Scenario 2: Compositing multiple structures}

A more complex use case involves fitting multiple structures to a single, large, often complex, volumetric dataset, such as assembling a viral capsid from individual protein units or constructing a ribosomal complex from its constituent proteins and RNA molecules. \acronym can manage such composite fitting tasks by iteratively optimizing the placement of each component, from largest to smallest, considering the spatial relationships and interactions between them to prevent overlaps and ensure a coherent assembly.

\autoref{fig:teaser} depicts an example of compositing multiple structures into a \ac{Cryo-em} volume map for the PDB-protein \href{https://doi.org/10.2210/pdb8SMK/pdb}{8SMK} \cite{Zhou:2024:ADI}. The first row demonstrates how the middle and bottom parts are fitted in the first computation round, with the remaining top part of the protein fitted in the second round of the interactive process.

The ability to \emph{zero-out} densities, once a fit is confirmed, allows \acronym to fit multiple structures sequentially without interference from previously placed components, as demonstrated in \autoref{fig:teaser}. This iterative approach is valuable for densely packed molecular complexes, where individual components may be difficult to distinguish in the volumetric data. This scenario is critical for understanding the functional context of proteins in larger biomolecular assemblies or cellular environments.

\subsection{Scenario 3: Identify unknown densities}

\acronym also offers bioscientists the capability to identify and characterize unknown densities within volumetric datasets. In cases where a volume contains unassigned or ambiguous regions, possibly indicating the presence of previously unidentified molecules or molecular complexes, \acronym can be used to screen a library of known structures and predicted structures for potential matches.

By fitting the structures from a library to the unidentified densities and evaluating the fit quality, researchers can hypothesize the identity of the unknown components. This scenario is invaluable for discovery-based research, where identifying novel components in complex molecular assemblies could lead to significant biological insights.

\begin{figure}
     \centering
     %\begin{subfigure}[b]{1.0\linewidth}
         %\centering
         \subfigure[Library of structures to search against (subset).]{\label{fig:use_scenario_3_library}\includegraphics[width=\columnwidth]{figs/use_scenario_3_1.png}}\\[1ex]
         %\caption{Library of structures to search against}
         %\label{fig:use_scenario_3_library}
     %\end{subfigure}
     %\hfill
     %\begin{subfigure}[b]{1.0\linewidth}
         %\centering
         \subfigure[Unknown density identification: comparison of three potential fits overlaid on  the target volumes.]{\label{fig:use_scenario_3_result}\includegraphics[width=\columnwidth]{figs/use_scenario_3_2.png}}\vspace{-2ex}
         %\caption{Search results; Left: the top hit, middle: a fair alignment, right: a bad alignment}
         %\label{fig:use_scenario_3_result}
     %\end{subfigure}
        \caption{Unknown density identification, where dozens to hundreds of molecular structures can be evaluated for potential fit.}\vspace{2ex}
        \label{fig:three graphs}
\end{figure}

A search was performed with the demonstration dataset from a recent automated domain-level protein identification technique, DomainFit \cite{Gao:2023:DIP}. The task was to identify which domains from a library of 359 protein domains (\autoref{fig:use_scenario_3_library} shows a subset) which one(s) best fit into the given volume (\autoref{fig:use_scenario_3_result}). DomainFit identified two candidates (I7MLV6\_D3, and I7M317\_D1) after fitting all domains using the \texttt{fitmap} command in ChimeraX and performed statistical analyses to remove false positives. These same two candidates were identified with the proposed fitting technique using \acronym followed by a visual inspection, where the two candidates were the first to be inspected. The hit times were reported the same as in \autoref{table:identify_unknown} to compare the approaches, showing a $\approx$\,2\texttimes\ gain on the hit rate. In addition, DomainFit takes approx.\ 12 h to finish the task, whereas \acronym takes $\approx$\,10 min---a 72\texttimes\ gain in computational time. 


\begin{table}[t]
\caption{Performance results for identifying unknown structures. C stands for ChimeraX, D stands for \acronym; Gain = D/C for Hit.\vspace{-1ex}}
\centering
\begin{tabu}{llll}
\toprule
Structure  & C Hit & D Hit & Gain \\
\midrule
I7MLV6\_D3 & 108   & 280   & 2.6\texttimes  \\
I7M317\_D1 & 127   & 163   & 1.3\texttimes  \\
\bottomrule
\end{tabu}
\label{table:identify_unknown}
%
%\vspace{1ex}C stands for ChimeraX, D stands for \acronym; Gain = D/C for Hit.
\end{table}


==> content/04.1-Evaluation.tex <==
\section{Feedback}

In addition to the quantitative metrics reported in the use cases above, qualitative feedback from users is crucial in evaluating the practical utility and user experience for \acronym. We thus solicited feedback from a diverse group of users, including PhD students, structural biologists, and computational scientists, through surveys, interviews, and hands-on testing sessions. Seven people responded to our request, and we report key themes from their qualitative feedback as follows.

\textbf{Usability.} The participants appreciated the intuitive interface and workflow  (``quite intuitive and easy to use'') of \acronym, which significantly lowers the barrier to entry for new users while providing advanced features for experienced researchers. The visually guided fitting process was highlighted as a powerful feature for refining fitting results based on expert judgment. Suggestions for further improvements of this interaction step were to display several visual clusters at a time, to visually compare the fit results, and to offer a tab-based method to check the various clusters. This approach would make it easier to observe how each cluster fits relative to the \ac{Cryo-em} volume; thus, researchers would be better able to focus on a chain of interest. 

\textbf{Effect on Research.} The participants reported that \acronym has the potential to have a tangible impact on their research, enabling them to address complex fitting challenges that were previously out of reach, such as the ability to rapidly sample a large database of candidate structures for regions with unassigned protein density. The new ability to fit structures rapidly and accurately into volumetric data offers new directions of investigation and has the potential to accelerate discoveries in structural biology. One respondent stated that the automatic fitting and visual inspection approach ``could be a key feature in ChimeraX that [could become] a standard in many pipelines'' and ``a key implementation [for] a standard modeling workflow.''

The respondents also made suggestions for future developments, such as better structuring the handling of the associated files and adding workflows that would require automatically creating model subdivisions and performing fits on those before integrating the results into the reference volume. They also highlighted further potential uses, such as employing the proposed approach to analyze density maps generated using X-ray crystallography.


==> content/04.2-Implementation.tex <==
\section{Implementation}
\label{sec:implementation}
We utilized \texttt{PyTorch} for the DiffFit algorithm implementation, capitalizing on its dynamic computational graph, automatic differentiation, and GPU acceleration to estimate positional offset and rotational quaternion parameters efficiently. Specifically, we employed \texttt{torch.nn.Conv3d} for Gaussian smoothing and \texttt{torch.nn.functional.grid\_sample} for trilinear interpolation with the padding mode set to ``border.'' 
This approach enables rapid processing of large volumes and multiple structures. 
We leveraged tensor operations and the Adam optimization algorithm for accurate optimization results. 
We also integrated additional functions from the \texttt{SciPy}, \texttt{Bio.PDB}, \texttt{mrcfile}, and \texttt{Numpy} libraries to enhance the functionality of the algorithm. In addition, \acronym was seamlessly integrated into ChimeraX (\autoref{fig:visual-browser}) based on its bundle development environment. 

==> content/05-Discussion-orig.tex <==
\section{Discussion}
\label{sec:discussion}

\todo{TI: I feel that the discussion and conclusion should be revised (and the ChatGPT lingo taken out); maybe Ivan could give it a pass and really extract the new contributions; potentially they could also be merged into a single section}

\acronym represents a significant advancement in the field of structural biology, offering an efficient and accurate method for protein structure determination. Its development underscores the potential of utilizing differentiable optimization algorithms within the domain, particularly for complex molecular structures. 

, coupled with its integration into established visualization tools like ChimeraX, signifies a step forward in accessibility and utility for researchers.



==> content/05-Discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\todo{TI: I feel that the discussion and conclusion should be revised (and the ChatGPT lingo taken out); maybe Ivan could give it a pass and really extract the new contributions; potentially they could also be merged into a single section}

\acronym represents a significant advancement in the field of structural biology, offering an efficient and accurate method for protein structure determination. Its development underscores the potential of utilizing differentiable optimization algorithms within the domain, particularly for complex molecular structures. 

, coupled with its integration into established visualization tools like ChimeraX, signifies a step forward in accessibility and utility for researchers.



==> content/06-Conclusion.tex <==
\section{Limitations and Future Work}
Although the proposed technique demonstrates substantial improvement over state-of-the-art techniques, it also has limitations. One issue arises in Scenario 2 due to the gradual \emph{zeroing-out} of the target map, where multiple structures are composited onto a single map. In this case, the volume removal could remove voxels that are part of adjacent interacting molecular subunits. Then, the subsequent subunit might have difficulty finding its correct location because these few zeroed voxels penalize the correct position. This limitation is being investigated, and we plan to experiment with heuristics that remove only voxels fully covered by the molecular structure or slightly shrink the to-be-\emph{zeroed-out} region before removing it from the map. Another related limitation is that the fitting process does not check for collisions in adjacent subunits, as previously investigated in visualization work (e.g., \cite{Schmidt:2014:YMCA}). Although the map-shrinking process should address this problem, in some cases, subunits may still overlap. This problem could be straightforwardly resolved by removing  subunit poses that overlap with previously confirmed subunit placements or by performing a minimal pose modification to resolve structural collisions.

The proposed technique is also not completely parameter-free, which would be ideal. The threshold value for removing voxels with small density values, for example, and the threshold value for the connected-voxel minimal cluster size must be manually set. Manipulating these parameters requires that bioscientists have prior domain experience with \ac{Cryo-em} data. We aim to automate the identification of these thresholds or at least define suitable default values and provide guidance on reasonable parameter ranges.

The visualization design in the current version of the tool also offers only the most essential visual encoding types, with a clear potential for further improvement. We plan to adapt comparative visualization techniques to intersect surfaces and smart visibility techniques for combined rendering of the volumetric density representation with molecular surfaces or cartoon representations. Furthermore, the visualization design for analyzing structural poses in a cluster suffers from high spatial occlusion of the subunit poses (see \autoref{fig:clustering_filtering:d}). This common domain problem requires a dedicated research effort to combat the occlusion of this magnitude.


Driven by the feedback, additional possible future research directions include extending \acronym to deformable transformations, considering stoichiometry and symmetry, and speedingit up by integration with CUDA.

\section{Conclusion}
\label{sec:conclusion}
In conclusion, DiffFit offers a novel and efficient solution to the challenges of atom-to-map fitting, which has recently arisen in structural biology. These challenges are addressed with the proposed differentiable fitting algorithm and a set of essential strategies that make the algorithm robust for the domain problem. The approach adds a human-in-the-loop visual analytics approach to the workflow and provides an open-source package designed to work as part of a standard software tool on the domain (ChimeraX).
A critical element of the proposed approach is the change from pixel-to-pixel (or the equivalent, voxel-to-voxel) fitting to point-to-volume fitting, enabling the management of the specific constraints of the fitting problem in structural biology.
The success of using atom coordinates to sample the volume instead of using all voxels suggests that, in the original technique that inspired our work \cite{Reddy2020Differentiable},  not all  pixels in a patch may be needed for the optimization. Thus, the image compositing optimization could be more efficient and could manage larger examples with faster processing. 

The reported quantitative performance metrics collectively demonstrate the substantial improvement of \acronym  over traditional approaches, highlighting its potential to transform the field of structural biology. This potential is high because the workflows of Assembline, a protocol published in 2022 \cite{Rantos:2022:ISM}, and DomainFit \cite{Gao:2023:DIP}, rely on the \texttt{fitmap} command on ChimeraX as the first step. This stage can be replaced by the more effective \acronym, offering a new foundation for these and other workflows.
By demonstrating the effectiveness of the proposed technique across three scenarios, from fitting individual structures to assembling complex molecular architectures and identifying unknown components, \acronym overcomes the limitations of manually placing individual molecules before fitting, making the compositing faster, more accurate, and intuitive and offering the possibility of scanning the entire set of known and predicted molecules with the current computational resources. Thus, the \href{https://en.wiktionary.org/wiki/Faustian_bargain}{Faustian bargain} \cite{Goethe:1808:F} is escaped, freeing researchers to explore the inner workings of the biological world.

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

